Programming-by-Demonstration for Long-Horizon Robot Tasks

The goal of programmatic Learning from Demonstration (LfD) is to learn a policy in a programming language that can be used to control a robot's behavior from a set of user demonstrations. This paper presents a new programmatic LfD algorithm that targets long-horizon robot tasks which require synthesizing programs with complex control flow structures, including nested loops with multiple conditionals. Our proposed method first learns a program sketch that captures the target program's control flow and then completes this sketch using an LLM-guided search procedure that incorporates a novel technique for proving unrealizability of programming-by-demonstration problems. We have implemented our approach in a new tool called PROLEX and present the results of a comprehensive experimental evaluation on 120 benchmarks involving complex tasks and environments. We show that, given a 120 second time limit, PROLEX can find a program consistent with the demonstrations in 80% of the cases. Furthermore, for 81% of the tasks for which a solution is returned, PROLEX is able to find the ground truth program with just one demonstration. In comparison, CVC5, a syntax guided synthesis tool, is only able to solve 25% of the cases even when given the ground truth program sketch, and an LLM-based approach, GPT-Synth, is unable to solve any of the tasks due to the environment complexity.

==> deprecated/fig_oper_sem.tex <==
\def\horizontalSpace{5mm}
\begin{figure}[t]
\footnotesize
\begin{minipage}[t]{0.24\textwidth}
  \ruleLabel{drop-ctx}
$$
\RULE{
\env, \Delta, \emptyset, c \xrightarrow{l}\env',\Delta', \_ \,, c'
}
%% ----------------------------------------------------------------
{
\env, \Delta, c \xrightarrow{l}\env',\Delta', c'
}
$$
\end{minipage}
\hfill
\begin{minipage}[t]{0.29\textwidth}
  \ruleLabel{sequence}
$$
\RULE{
\env, \Delta, \Sigma, c \xrightarrow{l}\env',\Delta', \Sigma', c''
}
%% ----------------------------------------------------------------
{
\env, \Delta, \Sigma, c;c' \xrightarrow{l}\env',\Delta', \Sigma', c'';c'
}
$$
\end{minipage}
\hfill
\begin{minipage}[t]{0.27\textwidth}
  \ruleLabel{skip}
$$
\RULE{
\\
}
%% ----------------------------------------------------------------
{
\env, \Delta, \Sigma, \stx{skip};c \xrightarrow{l}\env,\Delta, \Sigma, c
}
$$
\end{minipage}
\\[\horizontalSpace]
\begin{minipage}[t]{0.53\textwidth}
  \ruleLabel{scan}
$$
\RULE{
\env, \Delta;\demo{scan(t)}, \Sigma[\set{v}\mapsto \env.\mathtt{objs}(l,t)], c\xrightarrow{l}\env',\Delta', \_\,, \stx{skip}
}
%% ----------------------------------------------------------------
{
\env, \Delta, \Sigma, \stx{let}\; \set{v}:= \stx{scan}(t) \,\stx{in}\, \{c\}  \xrightarrow{l}\env',\Delta', \Sigma, \stx{skip}
}
$$
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\textwidth}
  \ruleLabel{choose}
$$
\RULE{
\env, \Delta, \Sigma[
v \mapsto \Sigma(\set{v})[n]], 
c\xrightarrow{l}\env',\Delta', \_\,, \stx{skip}
}
%% ----------------------------------------------------------------
{
\env, \Delta, \Sigma, \stx{let}\; v:= \set{v}[n] \,\stx{in}\, \{c\}  \xrightarrow{l}\env',\Delta', \Sigma, \stx{skip}
}
$$
\end{minipage}
\\[\horizontalSpace]
\begin{minipage}[t]{0.51\textwidth}
  \ruleLabel{iterate}
$$
\RULE{
\Delta_0 = \Delta 
\qquad
\env_0 = \env
\qquad 
n = |\Sigma(\set{v})|
\\
\forall_{0\leq i < n}.\; \env_i, \Delta_i, \Sigma[v\mapsto \Sigma(\set{v})[i]], c \
\xrightarrow{l} \env_{i+1}, \Delta_{i+1}, \_\, \stx{skip}
}
%% ----------------------------------------------------------------
{
\env, \Delta, \Sigma,
\stx{foreach} \;v\; \stx{in}\; \set{v}\; \stx{do}\; \{c\}
\xrightarrow{l}\env_n,\Delta_n, \Sigma, \stx{skip}
}
$$
\end{minipage}
\hfill
\begin{minipage}[t]{0.23\textwidth}
  \ruleLabel{if-t}
$$
\RULE{
\evalB{\phi}{ \env, \Sigma} =\top
\\
c = \stx{if} \;\phi\; \stx{then} \;\{c'\}  
}
%%  ----------------------------------------------------------------
{
\env, \Delta, \Sigma,c \xrightarrow{l}\env,\Delta, \Sigma, c'
}
$$
\end{minipage}
\hfill
\begin{minipage}[t]{.23\textwidth}
  \ruleLabel{if-f}
$$
\RULE{
\evalB{\phi}{ \env, \Sigma} = \bot
\\
c = \stx{if} \;\phi\; \stx{then} \;\{c'\} 
}
%% ----------------------------------------------------------------
{
\env, \Delta, \Sigma,c   \xrightarrow{l}\env,\Delta, \Sigma, \stx{skip}
}
$$
\end{minipage}
\\[\horizontalSpace]
\begin{minipage}[t]{0.49\textwidth}
  \ruleLabel{set-prop}
$$
\RULE{
o = \Sigma(v)
\\
\env' 
=(\env.\mathtt{locs},\env.\mathtt{objs},\env.\mathtt{props}[(o,p)\mapsto b],\env.\mathtt{rels})
}
%% ----------------------------------------------------------------
{
\env, \Delta, \Sigma, \stx{set\_prop}(v,p,b)  \xrightarrow{l}\env',\Delta;\demo{p(o)\!=\!b}, \Sigma, \stx{skip}
}
$$
\end{minipage}
\hfill
\begin{minipage}[t]{0.49\textwidth}
  \ruleLabel{set-rel}
$$
\RULE{
o_1 = \Sigma(v_1)
\qquad 
o_2 = \Sigma(v_2)
\\
\env' 
=(\env.\mathtt{locs},\env.\mathtt{objs},\env.\mathtt{props},\env.\mathtt{rels}[(o_1,o_2,r)\mapsto b])
}
%% ----------------------------------------------------------------
{
\env, \Delta, \Sigma, \stx{set\_rel}(v_1,v_2,r,b)  \xrightarrow{l}\env',\Delta;\demo{r(o_1,o_2)\!=\!b}, \Sigma, \stx{skip}
}
$$
\end{minipage}
\\[\horizontalSpace]
\begin{minipage}[t]{\textwidth}
  \ruleLabel{grab}
$$
\RULE{
o = \Sigma(v)
\qquad
t = \mathtt{type}(o)
\qquad
\mathtt{objs}' = \env.\mathtt{objs}[(l,t) \mapsto \env.\mathtt{objs}(l_\mathtt{R},t) \backslash \{v\}][(l_\mathtt{R},t) \mapsto \env.\mathtt{objs}(l_\mathtt{R},t) \cup \{v\}]
}
%%  ----------------------------------------------------------------
{
\env, \Delta, \Sigma,\stx{grab}(v)\xrightarrow{l}(\env.\mathtt{locs}, \mathtt{objs}', \env.\mathtt{props},\env.\mathtt{rels}),\Delta;\demo{grab(o)}, \Sigma, \stx{skip}
}
$$
\end{minipage}
\\[\horizontalSpace]
\begin{minipage}[t]{\textwidth}
  \ruleLabel{drop}
$$
\RULE{
o = \Sigma(v)
\qquad
t = \mathtt{type}(o)
\qquad
\mathtt{objs}' = \env.\mathtt{objs}[(l,t) \mapsto \env.\mathtt{objs}(l,t) \cup \{v\}][(l_\mathtt{R},t) \mapsto \env.\mathtt{objs}(l_\mathtt{R},t) \backslash \{v\}]
}
%% ----------------------------------------------------------------
{
\env, \Delta, \Sigma,\stx{drop}(v)\xrightarrow{l}(\env.\mathtt{locs}, \mathtt{objs}', \env.\mathtt{props},\env.\mathtt{rels}),\Delta;\demo{drop(o)}, \Sigma, \stx{skip}
}
$$
\end{minipage}

\caption{Auxiliary Semantics of Robot Executions in a Location $l$ (defined using $\xrightarrow{l}$ relation)}
\label{fig:operational_semantics}
\end{figure}


==> deprecated/fig_oper_sem_goto.tex <==
\def\horizontalSpace{5mm}
\begin{figure}[t]
\footnotesize
\begin{minipage}[t]{0.73\textwidth}
  \ruleLabel{goto-each}
$$
\RULE{
n = |\env.\mathtt{locs}|
\qquad 
\Delta_0 = \Delta
\qquad 
\env_0 = \env
\\
\forall_{0 \leq i < n}.\;  c_i = \stx{goto}[\env.\mathtt{locs}[i]]\{c\};\stx{done}
\qquad 
%\forall_{0 \leq i < n}.\;  \env_i, \Delta_i, c \xrightarrow{\env.\mathtt{locs}[i]}\env_{i+1},\Delta_{i+1}
%\\
\forall_{0 \leq i < n}.\; 
\env_i,\Delta_i,c_i
\,\Rightarrow \,
\env_{i+1}, \Delta_{i+1},\stx{done}
}
%% ----------------------------------------------------------------
{
\env,\Delta,\stx{goto\_each\_loc}\{c\};\pi
\,\Rightarrow \,
\env_n,\Delta_n,\pi
}
$$
\end{minipage}
\\[\horizontalSpace]
\begin{minipage}[t]{0.38\textwidth}
  \ruleLabel{goto}
$$
\RULE{
\env, \Delta;\demo{goto(l)}, c \xrightarrow{l}\env',\Delta',\stx{skip}
}
%% ----------------------------------------------------------------
{
\env,\Delta,\stx{goto}[l]\{c\};\pi
\,\Rightarrow \,
\env', \Delta',\pi
}
$$
\end{minipage}
\qquad
\begin{minipage}[t]{0.34\textwidth}
  \ruleLabel{done}
$$
\RULE{
\delta \not\eq \demo{done}
}
%% ----------------------------------------------------------------
{
\env, \Delta;\delta, \stx{done} \,\Rightarrow \, \env, \Delta;\delta;\demo{done}, \stx{done}
}
$$
\end{minipage}
\caption{Operational Semantics of Robot Execution Policies (defined using $\Rightarrow$ relation)}
\label{fig:operational_semantics}
\end{figure}


==> deprecated/history.tex <==
THIS FILE IS NOT INCLUDED IN THE PROJECT AND SIMPLY CONTAINS HISTORICAL CONTENTS THAT MAY BECOME USEFULL IN THE FUTTURE



The Behavior framework~\cite{pmlr-v164-srivastava22a}, as outlined in section~\ref{subsec:bench}, is a virtual environment that features a simulated embodied agent that can be controlled by humans using a VR headset or by a learned controller that dictates the agent's movements based on its observations.
%
The authors of Behavior evaluated the performance of  two state-of-the-art model-free reinforcement learning algorithms, on the benchmark's tasks, highlighting the challenges of this benchmark. 
The learned controllers used the agent's observations (such as RGB, depth, and proprioception) as input, and the policies were trained in the agent's original low-level continuous action space, as well as in high-level action primitives that were defined by the authors.
 %
%
In summary, their experiments revealed that the state-of-the-art embodied AI solutions face significant challenges with the complexity of the activities in Behavior. The learned agents were unable to accomplish \textit{any} of the goal conditions for even the simple tasks, and the authors highlight that the long-horizon nature of these activities is a critical challenge for reinforcement learning. 


\newpage



\begin{comment}
\subsection{\tool's Results}

In this section, we investigate the performance of \tool\ on the set of benchmark tasks presented earlier, as well as evaluate the efficacy of the infeasibility check and LLM guided enumeration through an ablation study. For this evaluation we consider the amount of time required to find a satisfying program for a given demonstration, the number of complete programs evaluated before satisfying a demonstration, and the rate at which \tool\ can successfully find a satisfying program. We also investigate the effect of increased difficulty of environments, as outlined in Table \ref{table:env}, and increased difficulty of demonstrations. In these experiments, demonstration difficulty is categorized by the amount of information not given by the end-user. An easy demonstration is missing 10\% of the maximum amount of information, a medium demonstration is missing 40\%, and a hard demonstration is missing 70\%. \todo{Kia: we need to clarify this.}

We first present the results of \tool\ grouped by task in Figure \ref{fig:prolex_res} for each pair of environment-demonstration difficulty. The top-left chart in Figure \ref{fig:prolex_res} shows the time in seconds required to find a solution using \tool\ for each triplet of task-environment-demonstration. As can be seen, \tool\ generally has higher performance on the easier environments and demonstrations, which is sensible as the enumeration space is smaller. \todo{$\leftarrow$ Is there anything more interesting to say here?}

The top right of Figure \ref{fig:prolex_res} shows the number of complete programs found by \tool\ before a satisfying program was discovered, for each pair environment-demonstration difficulty. \todo{Re-evaluate in the morning once multiple runs of medium environment take place to see if it's a stochasticity issue. Also re-run easy env since I don't think the seeding was occurring correctly.}

The bottom chart in Figure \ref{fig:prolex_res} shows the rate at which \tool\ was successful in finding a satisfying program, averaged over tasks, for each pair of environment-demonstration difficulty. As is shown, the easier environments and demonstrations have higher success rate as is to be expected. \todo{$\leftarrow$ Is there anything more interesting to say here?}



\begin{figure}[h]
    \centering
\begin{subfigure}[b]{\textwidth}
\centering
\includegraphics[width=0.9\textwidth]{Results/chart_time.png}
\caption{Time for completion for each benchmark categorized by the complexity of the environment and demo challenge level}
\label{subfig:time_plot}
\end{subfigure}

    
   % \includegraphics[width=0.48\textwidth]{Results/Prolex Time to Complete Across Demo and Env Difficulty.pdf}
   % ~
    \includegraphics[width=0.48\textwidth]{Results/Prolex Completions Checked Across Demo and Env Difficulty.pdf}
    ~
    \includegraphics[width=0.49\textwidth]{Results/Prolex Completion Rate Across Demo and Env Difficulty.pdf}
    
    \caption{Shows the results of running \tool\ on the benchmark tasks for each pair of difficulty of the demonstration and the environment. Top left shows time to find a satisfying program, top right shows complete programs checked before satisfying the demonstration, and bottom shows the success rate of finding a satisfying program.
    % TODO
    %
    % replace the groupings with color-coding
    % drop the .00 after the second values in y axis
    % x axis needs more labels to understand what is going on
    }
    \label{fig:prolex_res}
\end{figure}



%% ablation study

Now we present the results of our ablation study, showing the effect of each of the \tool's components in its overall performance. In particular, we define 3 variations of our full algorithm, namely LLM guided enumeration with no infeasibility check (No Inf Check), non-guided enumeration with infeasibility check (No LLM), and non-guided enumeration without infeasibility check (Vanilla). 

Figure \ref{fig:ablation_res} shows the results of the ablation study, using the same metrics that \tool\ was evaluated on previously. The top-left of Figure \ref{fig:ablation_res} shows the amount of time required in seconds for \tool\ and each of the three variations to find a result. As can be seen the performance of \tool\ outperform all the ablated versions except in rare instances where the overhead of checking for infeasibility provides a small downside in the amount of time taken. \todo{There is more to say here about the relative effects of LLM and inf checking}

The top-right chart of Figure \ref{fig:ablation_res} shows the number of complete programs evaluated before termination (in log scale) of \tool\ and the three ablated variations. This chart is averaged across all tasks and is grouped for each pair of environment-demonstration difficulty. \todo{Re-evaluate this after experiments mentioned above}

Lastly, the bottom of Figure \ref{fig:ablation_res} shows the rate at which each of the variations is able to successfully discover the correct program for each pair of environment-demonstration difficulty. As can be seen, \tool\ is most frequently able to find a satisfying program when compared to the three variations. As can be seen, when the enumeration space increases, the variations which do not use a language model to guide the search have success rates which drop off much quicker than the variations that do use language-model guided search, which lends credit to the effectiveness of the language model in guiding search.


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.48\textwidth]{Results/Average Ablated Completion Times Across Demo and Env Difficulty.pdf}
    ~
    \includegraphics[width=0.48\textwidth]{Results/Average Ablated Completions Checked Across Demo and Env Difficulty.pdf}
    
    \includegraphics[width=0.49\textwidth]{Results/Average Ablated Completion Rate Across Demo and Env Difficulty.pdf}
    \caption{Shows the results of running \tool\ and its ablated versions on the benchmark tasks for each pair of difficulty of the demonstration and the environment, where the results are averaged over the tasks. Top left shows time to find a satisfying program, top right shows complete programs checked before satisfying the demonstration, and bottom shows the success rate of finding a satisfying program.}
    \label{fig:ablation_res}
\end{figure}


The results discussed above show the effectiveness of LLM and inf check blah blah. 
Wrap up + Summary -> 
- tool is effective in general 
- performance suffers as the demos and envs become more comples. However, our LLM enable search suffers the least 


%% the stupid box :D :D 
\vspace{2mm}
\noindent\fbox{%
    \parbox{\textwidth}{%
    {\bf Summary. }
       Here we summarize the main results of this subsection for people who are lazy and will not read the whole thing. 
    }%
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{SyGuS Baseline}
Given a sketch for completing the task. Compare the solution finding of SyGus vs. our enumeration method.
\begin{enumerate}
    \item Chart showing time to completion of SyGus solution vs. our solution on easy/med/hard demos
    \item Chart showing time to completion of SyGus solution vs. our solution on easy/med/hard envs
    \item Chart showing percent correct (average over easy/med/hard env/demo) of SyGuS vs. our solution.
\end{enumerate}
%% the stupid box :D :D 
\vspace{2mm}
\noindent\fbox{%
    \parbox{\textwidth}{%
    {\bf Summary. }
       Here we summarize the main results of this subsection for people who are lazy and will not read the whole thing. 
    }%
}
\end{comment}



%final environment produced by running  and the resulting trace is identical to $\env'$. However, note that not all tasks performed in $\env$ can be fully specified by simply providing the final environment $\env'$. For instance, the final environment after executing the following two tasks is identical, even though the tasks themselves are different: 1) ``open the window; vacuum the room; close the window'' and 2) ``vacuum the room''. 
%
%As a result, our definition of the LfD challenge also ensures that the trace produced by executing $\pi^*$ on $\env$ is identical to $\trace$. More formally, we define 









%We also observed that particular re-orderings of program steps are semantic-preserving and do not affect successful execution of the task, hence, the target program $\pi^*$ does not need to produce the exact sequence of steps as $\trace$ when executed on $\env$. 

%
%To address the above observation, We introduce an equivalence relation (symbolized by $\equiv$) between execution traces that encapsulates what it means for a program to successfully perform a user-specified task. The equivalence relation is defined to admit 
%
 %For example, suppose the task is ``open the drawer, take a pen and a piece of paper from it, to the living room''. In this case, it is irrelevant whether the robot grabs the pen or paper first, as long as it eventually brings both to the living room.
%
%Conversely, specific steps are interdependent and must be completed in a particular order to successfully accomplish the task, for example, the robot must open the drawer before it can grab the pen and paper.
%
%For this reason, we ensure that $\equiv$ is strong enough to enforce such orderings between program steps that \emph{depend on each other}, and is relaxed enough to accept any order to performing the task steps, as long as the 



%Prior to formally defining $\equiv$, we first establish a dependency relation between objects that are manipulated during program execution.



%In particular, the equivalence relation is strong enough to ensure that two different trace which are equivalent traces indeed perform the

%and is weak enough to relax unnecessary ordering of events between unrelated items. ge addressed in this paper. 


%When a program $\pi$ is executed in an environment $\env$ and trace $\tau$ is produced, we say that $(\env,\trace)$ is a demonstration of the task performed by $\pi$. Our goal in this paper is to synthesize an unknown program $\pi^*$ given a small number of such demonstrations. We introduce the notation $(\env,\trace)\in\pi$, if and only if, 
%$\pi,\env,\sigma_0,\trace_0 \Rightarrow \stx{skip}, \_,\_,\trace$, where $\trace_0$ is an empty trace and $\sigma_0$ is an empty map.







%\begin{definition}
%\label{def:dep}
%\textit{Object Dependency in a Trace:} We define a "dependency"  relation between objects affected in an execution trace, as follows. Object $o$ and $o'$ are dependent if the trace contains either $\demo{acted(o,o',\_)}$ or $\demo{checked(o,o',\_)}$. We also each object is dependent on itself in all traces (reflexivity).
%\end{definition}


%\begin{definition}
%%\label{def:eq}
%\textit{Observational Equivalence of Traces:} We define two execution trace $\trace$ and $\trace'$ to be observationally equivalent, denoted by $\trace\equiv\trace'$, if and only if for all pairs of dependent objects $o$ and $o'$, the sequence of actions performed on $o$ and $o'$ in both traces are identical, i.e., $\forall_{o,o'}.\; dep(o,o')\Rightarrow 
 %\trace_{|o,o'} = \trace'_{|o,o'}$.
%\end{definition}

==> deprecated/temp.tex <==
\section{temp: old section 4}
We begin by presenting the top-level synthesis 
algorithm in \autoref{alg:top}. 



\subsection{Sketch Inference}
\begin{itemize}




    \item Alphabet of regular expressions
     \begin{mathpar}
  \begin{array}{lcl}
{r}  & := & 
 \demo{\mathcal{A}_{a,\tau_o}}
\ALT 
 \demo{\mathcal{A}_{a,\tau_o, \tau_o'}}
\ALT 
 \demo{\mathcal{G}_{\tau_l}}
\ALT 
  {rr}
 \ALT 
 {(r)^*} 
 \ALT 
 {(r)?} 
 \end{array}
  \end{mathpar}
%    \item function $learnRegex$: a black-box function that returns a set of regexes that \emph{all} accept the given strings. We can assume the returned set is ordered by complexity of the AST. 
  %  \item the language of sketches: similar to programs $\pi$ but allows holes ??.
 %   \item Translation of a regex to sketches
   \begin{comment} 
    \subitem 
    $\RULE{r\rhd s}{r\rhd \stx{let}\;v:= \stx{getNth}(\stx{scanObj}(??),??);s}$
       \qquad
    $\RULE{r\rhd s}{r\rhd \stx{let}\;v:= \stx{getNth}(\stx{scanLoc}(??),??);s}$
    
    \subitem\subitem
    $\RULE{r\rhd s}{(r)^*\rhd \stx{foreach}(v \in \stx{scanLoc}(??))\{s\}}$
    \quad
    $\RULE{r\rhd s}{(r)^*\rhd \stx{foreach}(v \in \stx{scanObj}(??))\{s\}}$ \quad $\RULE{r_1\rhd s_1\quad r_2\rhd s_2}{r_1 r_2 \rhd s_1;s_2}$
     \subitem\subitem
    $\RULE{r\rhd s}{ (r)? \rhd \stx{if}(??)\{s\}}$\quad $\RULE{}{\demo{\mathcal{A}_{a,\tau_o}} \rhd \stx{actUnary}(a, ??:\tau_o)}$
    \quad
    $\RULE{}{\demo{\mathcal{A}_{a,\tau_o, \tau'_o}} \rhd \stx{actBinary}(a, ??:\tau_o, ??:\tau'_o)}$ \subitem\subitem
    $\RULE{}{\demo{\mathcal{G}_{\tau_l}} \rhd \stx{goto}(??:\tau_l)}$

    %\subitem$\langle r_1 r_2\rangle := \langle r_1\rangle \langle r_2\rangle $
   % \subitem $\langle (r)?\rangle := \stx{if}(??)\{\langle r\rangle \}$
    %\subitem $\langle (r)^*\rangle := \stx{foreach}(v \in \stx{scanObj}(??))\{\langle r\rangle\}$ or $\stx{foreach}(v \in \stx{scanLoc}(??))\{\langle r\rangle\}$
    %\subitem $\langle \demo{\mathcal{A}_{a,\tau_o}} \rangle := \stx{actUnary}(a, ??:\tau_o)$
    %\subitem $\langle \demo{\mathcal{A}_{a,\tau_o, \tau'_o}} \rangle := \stx{actBinary}(a, ??:\tau_o, ??:\tau'_o)$
    %\subitem $\langle \demo{\mathcal{G}_{\tau_l}} \rangle := \stx{goto}(??:\tau_l)$

\end{comment}

\item Addition of scans to the manipulation-sketches: The above rules define a set of manipulation-sketches for each regex. A manipulation-sketch consists only of control structures and manipulation actions and does not include scans. For example, one of the manipulation-sketches derived from the regex (2) in \autoref{sec:mot}, is almost identical to the desired sketch shown in section 2, however, is missing line 3 which scans for bins


\item the order of sketch completion: scans -> acts -> if
\begin{comment}
\subitem  \begin{minipage}[b]{0.6\textwidth}
 \centering \footnotesize
\begin{mdframed}[backgroundcolor=grey12, linecolor=black,innerleftmargin=0mm]
  \begin{algorithmic}[1]
  {
  \STATE $\stx{foreach}(v_1\in \stx{scanLoc}(??))\{$
  \STATE  \ \ \  $\stx{goto}(??:room)^{\{room\}}$;
 % \STATE  \ \ \  $\stx{let}\; v_2:= \stx{getNth}(\stx{scanObj}(bed),0)$;
%   \STATE  \ \ \ $\stx{let}\; v_2:= \stx{getNth}(\stx{scanObj}(??),??)$;
   \STATE  \ \ \  $\stx{actUnary}(open, ??:bin)^{\{bin\}};$
  \STATE  \ \ \ $\stx{foreach}(v_2 \in \stx{scanObj}(??))\{$
  \STATE  \ \ \   \ \   $\stx{foreach}(v_3 \in \stx{scanObj}(??))\{$
  \STATE  \ \ \  \ \ \  \ \ \   $\stx{if}(??)\{$
    \STATE  \ \ \  \ \ \  \ \ \  \ \ \    $\stx{actUnary}(grab,??:sheet)^{\{sheet\}};$
      \STATE  \ \ \  \ \ \  \ \ \  \ \ \    $\stx{actBinary}(put\text{-}in,??:sheet,??:bin)^{\{sheet,bin\}};$
   \STATE  \ \ \  \ \ \  \ \ \ $\}$   
  \STATE  \ \ \   \ \   $\}$
  \STATE  \ \ \  $\}$
   \STATE  \ \ \   $\stx{actUnary}(close, ??:bin)^{\{bin\}};$
  \STATE $\}$
  }
 \end{algorithmic}
 \end{mdframed}
 \end{minipage}
\end{comment}

\end{itemize}


 \begin{definition}{\bf (Perception Completeness)}
 Consider a standard program order, $\prec$, between sketch statements.
 A sketch $s$ is defined to be perception complete, denoted as ${PC}(c)$, if and only if
 \begin{enumerate}
     \item for all statements $s_1:=\stx{actUnary}(a,??:\tau_o)$ in $s$, there exists a statement $s_2:=\stx{scanObj}(\tau_o)$, such that $s_2\prec s_1$.
     \item for all statements $s_1:=\stx{actBinary}(a,??:\tau_o,\tau'_o)$ in $s$, there exist statements $s_2:=\stx{scanObj}(\tau_o)$ and $s_3:=\stx{scanObj}(\tau'_o)$, such that $s_2\prec s_1$ and $s_3\prec s_1$.
     \item for all statements $s_1:=\stx{goto}(??:\tau_l)$ in $s$, there exists a statement $s_2:=\stx{scanLoc}(\tau_l)$ in $s$ such that $s_2\prec s_1$.
 \end{enumerate}
\end{definition}


We now define what it means for a sketch to be consistent with demonstration. This is used in line 7 of \autoref{alg:top}.




\newpage
\subsection{Sketch Completion}

%
%We finish this section by presenting our search algorithm for program completions parameterized by a black-box probabilistic model of program components. 
%
%In \autoref{sec:llm} we explain how to implement this model using a large language model, including our method of engineering prompts. 


%\subsection{Regex to Sketch Translation}
%Here we formally define how to translate a given regex that matches the demos, to an incomplete program (sketch).

%\subsection{Regex Expansion Rules}
%We explain why sometimes we need to consider different variations of a valid regex that

\begin{theorem}
(Completeness of Search) The inconsistency relation defined between sketches and demonstration traces is closed under hole completion, i.e., $\forall_{s,\delta}.\; s\not\sim \delta \Rightarrow \forall_{p\in\mathtt{completions}(s)}.\; p\not\sim \delta$.
\end{theorem}
%
The above theorem states that the our definition of sketch consistency with demonstrations 










==> fig_demo_trace_env.tex <==

\begin{figure}[t]
\footnotesize
\begin{subfigure}[b]{0.53\textwidth}
\centering
\begin{tabular}{|c|c|p{25mm}|c|}
\hline
Rooms & Beds     & \multicolumn{1}{c|}{Sheets}                                 & Bins      \\ \hline
r1    & bed1 & sheet1: \{on-bed, dirty\}, sheet2: \{on-bed, clean\}& bin1: \{closed\}  \\ \hline
r2    & bed2 & sheet3: \{on-bed, dirty\}, sheet4: \{on-bed, dirty\}             & bin2: \{closed\}   \\ \hline  
\end{tabular}
\\[4mm]
\begin{tabular}{|c|c|p{25mm}|c|}
\hline
Rooms & Beds     & \multicolumn{1}{c|}{Sheets}                                 & Bins      \\ \hline
r1    & bed1 & sheet1: \{in-bin, dirty\}, sheet2: \{on-bed, clean\}& bin1: \{closed\}  \\ \hline
r2    & bed2 & sheet3: \{in-bin, dirty\},  sheet4: \{in-bin, dirty\}             & bin2: \{closed\}   \\ \hline    
\end{tabular}
\caption{Partial representation of the environment before (top) and after (bottom) the demonstration. Only objects of interest and their states are shown.}
\label{subfig:demo_envs}
\end{subfigure}
%
\hfill
%
\begin{subfigure}[b]{0.38\textwidth}
\centering
\begin{minipage}[t]{\textwidth}
\[
\begin{array}{ll}
%\hspace{5mm} \demo{1\!:\!scan }\;\; \cmt{scan for rooms} \\ % location bedroom
\text{r1}
\begin{cases}
\ \demo{1\!:\!goto(r1)}\;\; \cmt{go to room1} \\ % go to first room
%\ \demo{3\!:\!scan}\;\; \cmt{scan for beds} \\ %  scan for bed
%\ \demo{4\!:\!scan}\;\; \cmt{scan for bins}\\ %  scan for bin
\ \demo{2\!:\!act(open, bin1)}\;\; \cmt{open bin1}\\ %  open bin
%\ \demo{6\!:\!scan}\;\; \cmt{scan for sheets}\\ % scan for clothes
%\ \demo{7\!:\!check}\;\; \cmt{check if sheet1 is clean}\\ % check the first clothe
\ \demo{3\!:\!act(grab, sheet1)}\;\; \cmt{grab sheet1}\\ % grab the first clothe
\ \demo{4\!:\!act(put\text{-}in, sheet1, bin1)}\;\; \cmt{put sheet1 in bin1}\\ % put the first clothe into the bin
%\ \demo{10\!:\!check}\;\; \cmt{check if sheet2 is clean}\\ % the second sheet was not dirty so there is no action performed% 
\ \demo{5\!:\!act(close, bin1)}\;\; \cmt{close bin1} %  close bin
\end{cases}
\end{array}
\]
\end{minipage}
\hfill
\begin{minipage}[t]{\textwidth}
\[
\begin{array}{ll}
\text{r2}
\begin{cases} 
\ \demo{6\!:\!goto(r2)}\;\; \cmt{go to room2} \\ % go to first room
%\ \demo{13\!:\!scan}\;\; \cmt{scan for beds}\\ %  scan for bed
%\ \demo{14\!:\!scan}\;\; \cmt{scan for bins}\\ %  scan for bin
\ \demo{7\!:\!act(open, bin2)}\;\; \cmt{open bin2}\\ %  open bin
%\ \demo{16\!:\!scan}\;\; \cmt{scan for sheets}\\ % scan for clothes
%\ \demo{17\!:\!check}\;\; \cmt{check if sheet3 is clean}\\ % check the first clothe
\ \demo{8\!:\!act(grab, sheet3)}\;\; \cmt{grab sheet3}\\ % grab the first clothe
\ \demo{9\!:\!act(put\text{-}in, sheet3, bin2)}\;\; \cmt{put sheet3 in bin2}\\ 
\ \demo{8\!:\!act(grab, sheet4)}\;\; \cmt{grab sheet4}\\ % grab the first clothe
\ \demo{9\!:\!act(put\text{-}in, sheet4, bin2)}\;\; \cmt{put sheet4 in bin2}\\ 
\ \demo{10\!:\!act(close, bin2)} \;\; \cmt{close bin2}%  close bin
\end{cases}
\end{array}
\]
\end{minipage}
\caption{Trace of demonstrated actions ($d$). %Commented texts (in grey color) are not part the input to the learner and are shown here only to assist the reader.
}
\label{subfig:demo_seq}
\end{subfigure}
    \caption{A demonstration  of the desired task in the running example. %consisting of a 
    %declaration of the environment (a) and a
    %sequence of the robot's actions (b).
    }
    \label{fig:demo}
\end{figure}


==> fig_demo_trace_env_2.tex <==

\begin{figure}[t]
\footnotesize
\begin{subfigure}[b]{0.83\textwidth}
\centering
\begin{tabular}{|c|p{95mm}|}
\hline
\textbf{Location} &\multicolumn{1}{c|}{\textbf{State}}   \\ \hline
$r_1$    &
\(
\begin{array}{lll}
  Objs & :  & \{lamp\!:\![l_1,l_2],\; bed\!:\![b_1],\; sheet\!:\![s_1, s_2],\; bin\!:\![bn_1],\dots \} \\
  Props  & :  & \{clean\!:\!\{s_2\},\; closed\!:\!\{bn_1\},\; off\!:\!\{l_1,l_2\}, \dots\}  \\
  Rels & : & \{on\text{-}top\!:\!\{(s_1,b_1),(s_2,b_1)\},\; next\text{-}to\!:\!\{(l_1,b_1),(l_2,b_1),\dots\},\\ & & \;\;inside\!:\!\{\},\dots\}  
\end{array}
\)   \\ \hline  
$r_2$    & \(
\begin{array}{lll}
  Objs & :  & \{lamp\!:\![l_3],\; bed\!:\![b_2],\; sheet\!:\![s_3, s_4],\; Bin\!:\![bn_2],\dots \} \\
  Props  & :  & \{clean\!:\!\{\},\; closed\!:\!\{bn_2\},\; off\!:\!\{l_3\},\dots\}  \\
  Rels & : & \{on\text{-}top\!:\!\{(s_3,b_2),(s_4,b_2)\},\; next\text{-}to\!:\!\{(l_3,b_2),\dots\},\\ & & 
  \;\;inside\{\},\dots\}  
\end{array}
\)     \\ \hline  
\end{tabular}
\\[4mm]
%%
%%
%%
%%
\caption{Partial representation of the initial environment. Only a small subset of objects, properties and relations are shown}
\label{subfig:demo_envs}
\end{subfigure}
%
\hfill
%
\begin{subfigure}[b]{0.38\textwidth}
\centering
\begin{minipage}[t]{\textwidth}
\[
\begin{array}{ll}
%\hspace{5mm} \demo{1\!:\!scan }\;\; \cmt{scan for rooms} \\ % location bedroom
\ \demo{1\!:\!goto(r_1)}\;\; \cmt{go to room1} \\ % go to first room
%\ \demo{3\!:\!scan}\;\; \cmt{scan for beds} \\ %  scan for bed
%\ \demo{4\!:\!scan}\;\; \cmt{scan for bins}\\ %  scan for bin
\ \demo{2\!:\!act(open, bn_1)}\;\; \cmt{open bin1}\\ %  open bin
%\ \demo{6\!:\!scan}\;\; \cmt{scan for sheets}\\ % scan for clothes
%\ \demo{7\!:\!check}\;\; \cmt{check if sheet1 is clean}\\ % check the first clothe
\ \demo{3\!:\!act(grab, s_1)}\;\; \cmt{grab sheet1}\\ % grab the first clothe
\ \demo{4\!:\!act(put\text{-}in, s_1, bn_1)}\;\; \cmt{put sheet1 in bin1}\\ % put the first clothe into the bin
%\ \demo{10\!:\!check}\;\; \cmt{check if sheet2 is clean}\\ % the second sheet was not dirty so there is no action performed% 
\ \demo{5\!:\!act(close, bn_1)}\;\; \cmt{closed bin1} \\%  closed bin\\
\ \demo{6\!:\!goto(r_2)}\;\; \cmt{go to room2} \\ % go to first room
%\ \demo{13\!:\!scan}\;\; \cmt{scan for beds}\\ %  scan for bed
%\ \demo{14\!:\!scan}\;\; \cmt{scan for bins}\\ %  scan for bin
\ \demo{7\!:\!act(open, bn_2)}\;\; \cmt{open bin2}\\ %  open bin
%\ \demo{16\!:\!scan}\;\; \cmt{scan for sheets}\\ % scan for clothes
%\ \demo{17\!:\!check}\;\; \cmt{check if sheet3 is clean}\\ % check the first clothe
\ \demo{8\!:\!act(grab, s_3)}\;\; \cmt{grab sheet3}\\ % grab the first clothe
\ \demo{9\!:\!act(put\text{-}in, s_3, bn_2)}\;\; \cmt{put sheet3 in bin2}\\ 
\ \demo{10\!:\!act(grab, s_4)}\;\; \cmt{grab sheet4}\\ % grab the first clothe
\ \demo{11\!:\!act(put\text{-}in, s_4, bn_2)}\;\; \cmt{put sheet4 in bin2}\\ 
\ \demo{12\!:\!act(close, bn_2)} \;\; \cmt{closed bin2}%  closed bin
\end{array}
\]
\end{minipage}
\caption{Trace of demonstrated actions ($d$).
%Commented texts (in grey color) are not part the input to the learner and are shown here only to assist the reader.
}
\label{subfig:demo_seq}
\end{subfigure}
    \caption{A demonstration  of the desired task in the running example. %consisting of a 
    %declaration of the environment (a) and a
    %sequence of the robot's actions (b).
    }
    \label{fig:demo}
\end{figure}



\begin{comment}
\begin{minipage}[t]{\textwidth}
\[
\begin{array}{ll}
%\hspace{5mm} \demo{1\!:\!scan }\;\; \cmt{scan for rooms} \\ % location bedroom
\text{r1}
\begin{cases}
\ \demo{1\!:\!goto(r1)}\;\; \cmt{go to room1} \\ % go to first room
%\ \demo{3\!:\!scan}\;\; \cmt{scan for beds} \\ %  scan for bed
%\ \demo{4\!:\!scan}\;\; \cmt{scan for bins}\\ %  scan for bin
\ \demo{2\!:\!act(open, bin1)}\;\; \cmt{open bin1}\\ %  open bin
%\ \demo{6\!:\!scan}\;\; \cmt{scan for sheets}\\ % scan for clothes
%\ \demo{7\!:\!check}\;\; \cmt{check if sheet1 is clean}\\ % check the first clothe
\ \demo{3\!:\!act(grab, sheet1)}\;\; \cmt{grab sheet1}\\ % grab the first clothe
\ \demo{4\!:\!act(put\text{-}in, sheet1, bin1)}\;\; \cmt{put sheet1 in bin1}\\ % put the first clothe into the bin
%\ \demo{10\!:\!check}\;\; \cmt{check if sheet2 is clean}\\ % the second sheet was not dirty so there is no action performed% 
\ \demo{5\!:\!act(closed, bin1)}\;\; \cmt{closed bin1} %  closed bin
\end{cases}
\end{array}
\]
\end{minipage}
\hfill
\begin{minipage}[t]{\textwidth}
\[
\begin{array}{ll}
\text{r2}
\begin{cases} 
\ \demo{6\!:\!goto(r2)}\;\; \cmt{go to room2} \\ % go to first room
%\ \demo{13\!:\!scan}\;\; \cmt{scan for beds}\\ %  scan for bed
%\ \demo{14\!:\!scan}\;\; \cmt{scan for bins}\\ %  scan for bin
\ \demo{7\!:\!act(open, bin2)}\;\; \cmt{open bin2}\\ %  open bin
%\ \demo{16\!:\!scan}\;\; \cmt{scan for sheets}\\ % scan for clothes
%\ \demo{17\!:\!check}\;\; \cmt{check if sheet3 is clean}\\ % check the first clothe
\ \demo{8\!:\!act(grab, sheet3)}\;\; \cmt{grab sheet3}\\ % grab the first clothe
\ \demo{9\!:\!act(put\text{-}in, sheet3, bin2)}\;\; \cmt{put sheet3 in bin2}\\ 
\ \demo{8\!:\!act(grab, sheet4)}\;\; \cmt{grab sheet4}\\ % grab the first clothe
\ \demo{9\!:\!act(put\text{-}in, sheet4, bin2)}\;\; \cmt{put sheet4 in bin2}\\ 
\ \demo{10\!:\!act(closed, bin2)} \;\; \cmt{closed bin2}%  closed bin
\end{cases}
\end{array}
\]
\end{minipage}
\end{comment}

==> fig_expr_reduction.tex <==
\begin{comment}
\begin{figure}[t]
\footnotesize
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{minipage}{\textwidth}
 \begin{mathpar}
 \begin{array}{lcl}
 \evalB{\stx{check\_prop}(prop,v)}{\env,\Sigma} & := & \env.\mathtt{props}(\Sigma(v),prop), \demo{checked(prop,\Sigma(v))} \\
 \evalB{\stx{check\_rel}(rel,v,v')}{\env,\Sigma} & := & \env.\mathtt{rels}(\Sigma(v),\Sigma(v'),rel), \demo{checked(rel,\Sigma(v),\Sigma(v'))} \\
 \evalB{c\wedge c'}{\env,\Sigma} & := &  ?? \\
\evalB{c\vee c'}{\env,\Sigma} & := &  ?? \\
\evalB{\neg c}{\env,\Sigma} & := &  ?? 
 \end{array}
 \end{mathpar}
 \end{minipage}
  \caption{Boolean Expression Reduction (defined using $\evalB{.}{}$ function parameterized by $\env$ and $\Sigma$)}
  \label{fig:bool_expression_reduction}
\end{figure}
\end{comment}

==> fig_llm.tex <==
\begin{figure}[h]
    \footnotesize
    \begin{flalign*}
    &
    \text{LLM Prompt}
        \begin{cases}
 \texttt{TBD}
    \end{cases} \\
    &
            \text{LLM Output}
        \begin{cases}
 \texttt{TBD}
    \end{cases}
    \end{flalign*}
     
    \caption{The LLM prompt (top) and its output (bottom).}
    \label{fig:llm}
\end{figure}

==> fig_motiv_ex.tex <==
\algsetup{
    linenosize=\Small,
    linenodelimiter = {:}
}

\begin{figure}[t]
\scriptsize
\begin{subfigure}[b]{0.56\textwidth}
\begin{mdframed}[backgroundcolor=white, linecolor=black,innerleftmargin=0mm]
 \begin{algorithmic}[1]
  {

  \STATE $\stx{foreach}(v_1\in \stx{scanLoc}(room))\{$
  \STATE  \ \ \   $\stx{goto}(v_1)$;
 % \STATE  \ \ \  $\stx{let}\; v_2:= \stx{getNth}(\stx{scanObj}(bed),0)$;
   \STATE  \ \ \  $\stx{let}\; v_2:= \stx{getFirst}(\stx{scanObj}(bin))$;
   \STATE  \ \ \   $\stx{actUnary}(open, v_2);$
  \STATE  \ \ \  $\stx{foreach}(v_3 \in \stx{scanObj}(bed))\{$
  \STATE  \ \ \   \ \ \   $\stx{foreach}(v_4 \in \stx{scanObj}(sheet))\{$
  \STATE  \ \ \  \ \ \  \ \ \  \ \ $\stx{if}(\stx{checkProp}(dirty, v_4) \wedge$ $\stx{checkRel}(on\text{-}top\text{-}of, v_4,v_3))\{$
   % \\  \ \ \  \ \ \  \ \ \  \ \ \  \ \ \ \ \ \ \ \ \ \ \ $\stx{checkRel}(on\text{-}top\text{-}of, v_4,v_3))\{$
    
    \STATE  \ \ \  \ \ \  \ \ \  \ \ \  \ \ \   $\stx{actUnary}(grab,v_4);$
    \STATE  \ \ \  \ \ \  \ \ \  \ \ \  \ \ \  \hspace{-1mm} $\stx{actBinary}(put\text{-}in,v_4,v_2);$
   \STATE  \ \ \  \ \ \  \ \ \  \ \ $\}$   
  \STATE  \ \ \   \ \ \   $\}$
  \STATE  \ \ \  $\}$%$\}$$\}$
   \STATE  \ \ \   $\stx{actUnary}(close, v_2);$
  \STATE $\}$
  }
 \end{algorithmic}
 \end{mdframed}
   \caption{Ground-truth robot program}
 \label{subfig:gt}
 \end{subfigure}
 \hfill
 \begin{subfigure}[b]{0.43\textwidth}
 \centering
\begin{mdframed}[ linecolor=black,innerleftmargin=0mm]
  \begin{algorithmic}[1]
  {

  \STATE $\stx{foreach}(v_1\in \stx{scanLoc}(??))\{$
  \STATE  \ \ \  $\stx{goto}(??:room)$;
 % \STATE  \ \ \  $\stx{let}\; v_2:= \stx{getNth}(\stx{scanObj}(bed),0)$;
   \STATE  \ \ \ $\stx{let}\; v_2:= \stx{getFirst}(\stx{scanObj}(??))$;
   \STATE  \ \ \  $\stx{actUnary}(open, ??:bin);$
  \STATE  \ \ \ $\stx{foreach}(v_3 \in \stx{scanObj}(??))\{$
  \STATE  \ \ \   \ \   $\stx{foreach}(v_4 \in \stx{scanObj}(??))\{$
  \STATE  \ \ \  \ \ \  \ \ \   $\stx{if}(??)\{$
    \STATE  \ \ \  \ \ \  \ \ \  \ \ \    $\stx{actUnary}(grab,??:sheet);$
      \STATE  \ \ \  \ \ \  \ \ \  \ \ \    $\stx{actBinary}(put\text{-}in,??:sheet,??:bin);$
   \STATE  \ \ \  \ \ \  \ \ \ $\}$   
  \STATE  \ \ \   \ \   $\}$
 \STATE  \ \ \  $\}$%$\}$$\}$
   \STATE  \ \ \   $\stx{actUnary}(close, ??:bin);$
  \STATE $\}$
  }
 \end{algorithmic}
 \end{mdframed}
   \caption{Inferred sketch}
   \label{subfig:sketch}
 \end{subfigure}
 \hfill
 \begin{subfigure}[b]{0.43\textwidth}
 \centering
\begin{mdframed}[ linecolor=black,innerleftmargin=0mm]
  \begin{algorithmic}[1]
  {

  \STATE $\stx{foreach}(v_1\in \stx{scanLoc}(room))\{$
  \STATE  \ \ \  $\stx{goto}(??:room)$;
 % \STATE  \ \ \  $\stx{let}\; v_2:= \stx{getNth}(\stx{scanObj}(bed),0)$;
   \STATE  \ \ \ $\stx{let}\; v_2:= \stx{getFirst}(\stx{scanObj}(??))$;
   \STATE  \ \ \  $\stx{actUnary}(open, ??:bin);$
  \STATE  \ \ \ $\stx{foreach}(v_3 \in \stx{scanObj}(??))\{$
  \STATE  \ \ \   \ \   $\stx{foreach}(v_4 \in \stx{scanObj}(sheet))\{$
    \STATE  \ \ \  \ \ \  \ \ \  $\stx{actUnary}(grab,??:sheet);$
      \STATE  \ \ \  \ \ \  \ \ \   $\stx{actBinary}(put\text{-}in,??:sheet,??:bin);$
  \STATE  \ \ \   \ \   $\}$
 \STATE  \ \ \  $\}$%$\}$$\}$
   \STATE  \ \ \   $\stx{actUnary}(close, ??:bin);$
  \STATE $\}$
  }
 \end{algorithmic}
 \end{mdframed}
   \caption{Inferred sketch}
   \label{subfig:sketch}
 \end{subfigure}


\begin{subfigure}[b]{\textwidth}
% environment description
% we have 2 bedrooms
% in br1: 3 clothes and 2 of them satisfy the selection criteria
% in br2: 2 clothes and none satisfies the criteria 
 \label{subfig:demo}
 \end{subfigure}
    \caption{A robot program and the inferred sketch for it}
    \label{fig:motiv_ex}
\end{figure}





==> fig_trace.tex <==

\begin{figure}[t]
\footnotesize
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \begin{mathpar}
  \begin{array}{lcl}
\demo{\trace}  & := & 
 \demo{scanned(o)}
 \ALT 
  \demo{scanned(l)}
 \ALT 
 \demo{checked(p,\hat{o})} 
 \ALT 
 \demo{checked(r,\hat{o_1},\hat{o_2})} 
 \\ & & 
 \demo{acted(a,\hat{o})} 
 \ALT 
 \demo{acted(a,\hat{o_1},\hat{o_2})} \ALT 
 \demo{went\_to(\hat{l})}\ALT
 \demo{\trace};\demo{\trace} 
 \end{array}
  \end{mathpar}
  \caption{Syntax of Execution Traces. Object and location \emph{instances} are denoted with $\hat{}$ (hat).
  %\todo{Q: is it okay to have separate tokens for rel and prop checking? There is implicit information in  them which can help the enumeration.}
  }
  \label{fig:demo_syntax}
\end{figure}

==> learned_regexes.tex <==

\begin{figure}[b]
\footnotesize
\begin{comment}
\begin{subfigure}[b]{\textwidth}
\centering
$\begin{array}{ll}
\demo{\mathcal{S}_0}. % location bedroom
\demo{\mathcal{W}_{room}}.  % go to first room
\demo{\mathcal{S}_1}.  %  scan for bed
\demo{\mathcal{S}_2}.  %  scan for bin
\demo{\mathcal{A}_{open,bin}}.  %  open bin
\demo{\mathcal{S}_3}.  % scan for clothes
\demo{\mathcal{C}_0}.  % check the first clothe
\demo{\mathcal{A}_{grab,sheet}}.  % grab the first clothe
\demo{\mathcal{A}_{put,sheet,bin}}.  % put the first clothe into the bin
\demo{\mathcal{C}_0}.  % the second sheet was not dirty so there is no action performed% 
\demo{\mathcal{A}_{close,bin}}\;.\\ %  close bin
%%%%
\hspace{4.3mm}
\demo{\mathcal{W}_{room}}.  % go to first room
\demo{\mathcal{S}_1}.  %  scan for bed
\demo{\mathcal{S}_2}.  %  scan for bin
\demo{\mathcal{A}_{open,bin}}.  %  open bin
\demo{\mathcal{S}_3}.  % scan for clothes
\demo{\mathcal{C}_0}.  % check the first clothe
\demo{\mathcal{A}_{grab,sheet}}.  % grab the first clothe
\demo{\mathcal{A}_{put,sheet,bin}}.  
\demo{\mathcal{A}_{close,bin}} %  close bin

\end{array}$
\caption{string encoding of the demonstration}
\end{subfigure}
\end{comment}
%\\[6mm]
%\begin{subfigure}[b]{\textwidth}
\centering
\begin{tabular}{|c|l|}
\hline Mutation Rules
 & Regular Expression \\ 
\hline
- & $\demo{\mathcal{S}_0}(\demo{\mathcal{W}_{room}}\demo{\mathcal{S}_1}\demo{\mathcal{S}_2}\demo{\mathcal{A}_{open,bin}}\demo{\mathcal{S}_3}(\demo{\mathcal{C}_0}|\demo{\mathcal{A}_{grab,sheet}}|\demo{\mathcal{A}_{put,sheet,bin}})^*\demo{\mathcal{A}_{close,bin}})^*$\\ 
%
\hline
%
$(x|y|...)^*\rightarrow (xy...)^*$  & $\demo{\mathcal{S}_0}(\demo{\mathcal{W}_{room}}\demo{\mathcal{S}_1}\demo{\mathcal{S}_2}\demo{\mathcal{A}_{open,bin}}\demo{\mathcal{S}_3}(\demo{\mathcal{C}_0}\demo{\mathcal{A}_{grab,sheet}}\demo{\mathcal{A}_{put,sheet,bin}})^*\demo{\mathcal{A}_{close,bin}})^*$\\ 
%
\hline
%
$(x|y|...)^*\rightarrow (x(y...)?)^*$  & $\demo{\mathcal{S}_0}(\demo{\mathcal{W}_{room}}\demo{\mathcal{S}_1}\demo{\mathcal{S}_2}\demo{\mathcal{A}_{open,bin}}\demo{\mathcal{S}_3}(\demo{\mathcal{C}_0}(\demo{\mathcal{A}_{grab,sheet}}\demo{\mathcal{A}_{put,sheet,bin}})?)^*\demo{\mathcal{A}_{close,bin}})^*$\\ 
%
\hline
\end{tabular}
%\caption{learned regex}
%\end{subfigure}

    \caption{The expression learned from one of the string encodings of the demonstration  (first row)  and two of its mutations (second and third row). The third row contains the expression corresponding to the target sketch.}
    \label{fig:learned_regex}
\end{figure}


==> temp_guide_for_section_2.tex <==
\newpage
\section{temp: material for motivating example and overview}
Here are algorithms and other material to be used in section 2. 

\subsection{Robot-human}


\subsection{Sketch Inference Algorithm} % the full details will be presented in section 4
\begin{itemize}
    \item The language of demos: is similar to what we have in section 2, however, we do not need to include $\demo{check}$ in the trace any more.
    
    
    \item the updated environment needs to have one more dirty sheet on the bed in r2
    
    \begin{tabular}{|c|c|c|c|}
\hline
Rooms & Beds     & \multicolumn{1}{c|}{Sheets}                                 & Bins      \\ \hline
r1    & bed1 & sheet1: \{on-bed, dirty\}, sheet2: \{on-bed, clean\}& bin1: \{closed\}  \\ \hline
r2    & bed2 & sheet3: \{on-bed, dirty\} sheet4: \{on-bed, dirty\}                & bin2: \{closed\}   \\ \hline  
\end{tabular}
\\[4mm]
\begin{tabular}{|c|c|c|c|}
\hline
Rooms & Beds     & \multicolumn{1}{c|}{Sheets}                                 & Bins      \\ \hline
r1    & bed1 & sheet1: \{in-bin, dirty\}, sheet2: \{on-bed, clean\}& bin1: \{closed\}  \\ \hline
r2    & bed2 & sheet3: \{in-bin, dirty\} sheet4: \{in-bin, dirty\}              & bin2: \{closed\}   \\ \hline    
\end{tabular}
    
    \item The updated demo for the running example is given below. 
\[
\begin{array}{ll}
%\hspace{5mm} \demo{1\!:\!scan_l }\;\; \cmt{scan for rooms} \\ % location bedroom
\text{r1}
\begin{cases}
\ \demo{2\!:\!goto(r1)}\;\; \cmt{go to room1} \\ % go to first room
%\ \demo{3\!:\!scan_o}\;\; \cmt{scan for beds} \\ %  scan for bed
%\ \demo{4\!:\!scan_o}\;\; \cmt{scan for bins}\\ %  scan for bin
\ \demo{5\!:\!act(open, bin1)}\;\; \cmt{open bin1}\\ %  open bin
%\ \demo{6\!:\!scan_o}\;\; \cmt{scan for sheets}\\ % scan for clothes
%\ \demo{7\!:\!check}\;\; \cmt{check if sheet1 is clean}\\ % check the first clothe
\ \demo{7\!:\!act(grab, sheet1)}\;\; \cmt{grab sheet1}\\ % grab the first clothe
\ \demo{8\!:\!act(put\text{-}in, sheet1, bin1)}\;\; \cmt{put sheet1 in bin1}\\ % put the first clothe 
%\ \demo{10\!:\!check}\;\; \cmt{check if sheet2 is clean}\\ % the second sheet was not dirty so there is no action performed% 
\ \demo{9\!:\!act(close, bin1)}\;\; \cmt{close bin1} %  close bin
\end{cases}
\end{array}
\]
\\
\[
\begin{array}{ll}
\text{r2}
\begin{cases} 
\ \demo{10\!:\!goto(r2)}\;\; \cmt{go to room2} \\ % go to first room
%\ \demo{11\!:\!scan_o}\;\; \cmt{scan for beds}\\ %  scan for bed
%\ \demo{12\!:\!scan_o}\;\; \cmt{scan for bins}\\ %  scan for bin
\ \demo{13\!:\!act(open, bin2)}\;\; \cmt{open bin2}\\ %  open bin
%\ \demo{14\!:\!scan_o}\;\; \cmt{scan for sheets}\\ % scan for clothes
%\ \demo{17\!:\!check}\;\; \cmt{check if sheet3 is clean}\\ % check the first clothe
\ \demo{15\!:\!act(grab, sheet3)}\;\; \cmt{grab sheet3}\\ % grab the first clothe
\ \demo{16\!:\!act(put\text{-}in, sheet3, bin2)}\;\; \cmt{put sheet3 in bin2}\\ 
\ \demo{17\!:\!act(grab, sheet4)}\;\; \cmt{grab sheet4}\\ % grab the first clothe
\ \demo{18\!:\!act(put\text{-}in, sheet4, bin2)}\;\; \cmt{put sheet4 in bin2}\\ 
\ \demo{19\!:\!act(close, bin2)} \;\; \cmt{close bin2}%  close bin
\end{cases}
\end{array}
\]


    
    \item The string encoding: the encoded string of the above demo is:
    \[
\begin{array}{ll}
%\demo{\mathcal{S}_l}\, % location bedroom
\demo{\mathcal{G}_{room}}\,  % go to first room
%\demo{\mathcal{S}_o}\,  %  scan for bed
%\demo{\mathcal{S}_o}\,  %  scan for bin
\demo{\mathcal{A}_{open,bin}}\,  %  open bin
%\demo{\mathcal{S}_o}\,  % scan for clothes
%\demo{\mathcal{C}_0}\,  % check the first clothe
\demo{\mathcal{A}_{grab,sheet}}\,  % grab the first clothe
\demo{\mathcal{A}_{put,sheet,bin}}\,  % put the first clothe into the bin
%\demo{\mathcal{C}_0}\,  % the second sheet was not dirty so there is no action performed% 
\demo{\mathcal{A}_{close,bin}}\\ %  close bin
%%%%
%\hspace{4.4mm}
\demo{\mathcal{G}_{room}}\,  % go to first room
%\demo{\mathcal{S}_o}\,  %  scan for bed
%\demo{\mathcal{S}_o}\,  %  scan for bin
\demo{\mathcal{A}_{open,bin}}\,  %  open bin
%\demo{\mathcal{S}_o}\,  % scan for clothes
%\demo{\mathcal{C}_0}\,  % check the first clothe
\demo{\mathcal{A}_{grab,sheet}}\,  % grab the first clothe
\demo{\mathcal{A}_{put,sheet,bin}}\,  
\demo{\mathcal{A}_{grab,sheet}}\,  % grab the first clothe
\demo{\mathcal{A}_{put,sheet,bin}}\,  
\demo{\mathcal{A}_{close,bin}} %  close bin
\end{array}
\]

\item The encoding rules are trivial. The only thing is that we drop object/location instances and carry forward object/location types.


\item in the presentation here we are assuming the scans for locations and objects use different symbols both in the demo and in the string encoding. We can relax this assumption by using some very domain-specific knowledge about the programs and assume usage of the same symbol for both types of scans. In particular, we can limit scan of locations to happen only before gotos [more details should be figured out if we are going this route]. 



    \item The regex learner: given the string encoding will return a set of regexes. The first one shown below is the correct one but we show a few more which are valid:
    \[
%\demo{\mathcal{S}_l} % location bedroom
(\demo{\mathcal{G}_{room}}  % go to first room
%\demo{\mathcal{S}_o}  %  scan for bed
%\demo{\mathcal{S}_o}  %  scan for bin
\demo{\mathcal{A}_{open,bin}}  %  open bin
%\demo{\mathcal{S}_o}  % scan for clothes
%\demo{\mathcal{C}_0}\,  % check the first clothe
(\demo{\mathcal{A}_{grab,sheet}}  % grab the first clothe
\demo{\mathcal{A}_{put,sheet,bin}})^*  % put the first clothe into the bin
%\demo{\mathcal{C}_0}\,  % the second sheet was not dirty so there is no action performed% 
\demo{\mathcal{A}_{close,bin}}
)^*
\]
    \[
%\demo{\mathcal{S}_l} % location bedroom
(\demo{\mathcal{G}_{room}}  % go to first room
%\demo{\mathcal{S}_o}  %  scan for bed
%\demo{\mathcal{S}_o}  %  scan for bin
\demo{\mathcal{A}_{open,bin}}  %  open bin
%\demo{\mathcal{S}_o}  % scan for clothes
%\demo{\mathcal{C}_0}\,  % check the first clothe
((\demo{\mathcal{A}_{grab,sheet}}  % grab the first clothe
\demo{\mathcal{A}_{put,sheet,bin}})?)^*  % put the first clothe into the bin
%\demo{\mathcal{C}_0}\,  % the second sheet was not dirty so there is no action performed% 
\demo{\mathcal{A}_{close,bin}}
)^*
\]

    \[
%\demo{\mathcal{S}_l} % location bedroom
(\demo{\mathcal{G}_{room}}  % go to first room
%\demo{\mathcal{S}_o}  %  scan for bed
%\demo{\mathcal{S}_o}  %  scan for bin
(\demo{\mathcal{A}_{open,bin}})?  %  open bin
%\demo{\mathcal{S}_o}  % scan for clothes
%\demo{\mathcal{C}_0}\,  % check the first clothe
((\demo{\mathcal{A}_{grab,sheet}}  % grab the first clothe
\demo{\mathcal{A}_{put,sheet,bin}})?)^*  % put the first clothe into the bin
%\demo{\mathcal{C}_0}\,  % the second sheet was not dirty so there is no action performed% 
\demo{\mathcal{A}_{close,bin}}
)^*
\]

\begin{comment}
   \[
\demo{\mathcal{S}} % location bedroom
(\demo{\mathcal{G}_{room}}  % go to first room
\demo{\mathcal{S}}^*  %  scan for bed%  scan for bin
\demo{\mathcal{A}_{open,bin}}  %  open bin
\demo{\mathcal{S}}  % scan for clothes
%\demo{\mathcal{C}_0}\,  % check the first clothe
(\demo{\mathcal{A}_{grab,sheet}}|  % grab the first
\demo{\mathcal{A}_{put,sheet,bin}})^*  % put the first clothe into the bin
%\demo{\mathcal{C}_0}\,  % the second sheet was not dirty so there is no action performed% 
\demo{\mathcal{A}_{close,bin}}
)^*
\]


\item \textbf{Handling conditionals:} The learned regexes may not correctly capture the conditional structure of the target program. This is because, \dots. 


\subitem Our solution is to consider each $\demo{\mathcal{A}_{...}}$ independently, and see if we should add a ? after it. Later on, we analyze the rewritten expressions (or sketches) and try to merge consecutive ?s if possible, e.g. $A?B?$ can be turned into $(AB)?$. 


\subitem The first step is to identify the set of objects (or object pairs for binary actions), that could potentially be acted on given the current looping structure of the sketch 


We define a boolean function $F$ that given one of these $\demo{\mathcal{A}_{...}}$ , tells us whether it is conditionaled or not. 
\subitem The function $F$ first looks at the loops that are enclosing the given $\demo{\mathcal{A}_{...}}$. If there are Kleene * around it, it first 



\subitem 




%The regex learners are unable to identify conditionals -- because the Kleene star itself accepts zero or many instances of the enclosed actions. 





Assuming we can acquire  at least 2 distinguishing executions of some sequence of actions, A1A2...An we update the learned sketch by adding an if around the sequence, i.e. if(??){A1A2...An}. We define a function DISTINGUISH(A1A2...An, given\_demos) which decides if the sequence of actions Ai are always executed or not. When we say always, it could mean across iterations of an object loop, iterations of a location loop, or across different demonstrations. 

\item Using the above function, we update the regexes to become more precise and include The Match-zero-or-one Operator (?). Hence the above regexes will be rewritten to:

   \[
\demo{\mathcal{S}_l} % location bedroom
(\demo{\mathcal{G}_{room}}  % go to first room
\demo{\mathcal{S}_o}  %  scan for bed
\demo{\mathcal{S}_o}  %  scan for bin
\demo{\mathcal{A}_{open,bin}}  %  open bin
\demo{\mathcal{S}_o}  % scan for clothes
%\demo{\mathcal{C}_0}\,  % check the first clothe
((\demo{\mathcal{A}_{grab,sheet}}  % grab the first clothe
\demo{\mathcal{A}_{put,sheet,bin}})?)^*  % put the first clothe into the bin
%\demo{\mathcal{C}_0}\,  % the second sheet was not dirty so there is no action performed% 
\demo{\mathcal{A}_{close,bin}}
)^*
\]
   \[
\demo{\mathcal{S}_l} % location bedroom
(\demo{\mathcal{G}_{room}}  % go to first room
\demo{\mathcal{S}_o}^*  %  scan for bed%  scan for bin
\demo{\mathcal{A}_{open,bin}}  %  open bin
\demo{\mathcal{S}_o}  % scan for clothes
%\demo{\mathcal{C}_0}\,  % check the first clothe
((\demo{\mathcal{A}_{grab,sheet}}  % grab the first clothe
\demo{\mathcal{A}_{put,sheet,bin}})?)^*  % put the first clothe into the bin
%\demo{\mathcal{C}_0}\,  % the second sheet was not dirty so there is no action performed% 
\demo{\mathcal{A}_{close,bin}}
)^*
\]

   \[
\demo{\mathcal{S}} % location bedroom
(\demo{\mathcal{G}_{room}}  % go to first room
\demo{\mathcal{S}}^*  %  scan for bed%  scan for bin
\demo{\mathcal{A}_{open,bin}}  %  open bin
\demo{\mathcal{S}}  % scan for clothes
%\demo{\mathcal{C}_0}\,  % check the first clothe
(\demo{\mathcal{A}_{grab,sheet}}|  % grab the first
\demo{\mathcal{A}_{put,sheet,bin}})^*  % put the first clothe into the bin
%\demo{\mathcal{C}_0}\,  % the second sheet was not dirty so there is no action performed% 
\demo{\mathcal{A}_{close,bin}}
)^*
\]
\end{comment}



    \item The regex to sketch translation (returns a set of sketches):
    \subitem $[(x)^*] = \{\stx{foreach}(v\in \stx{scanLoc}(??))\{x'\} \;|\; x'\in[x]\} \cup \{\stx{foreach}(v\in \stx{scanObj}(??))\{x'\}\;|\; x'\in[x]\}$
    %\subitem [$\demo{\mathcal{S}_l}(x)^*$] = $\stx{foreach}(v\in \stx{scanLoc}(??))\{[x]\}$
     %\subitem [$\demo{\mathcal{S}_o}(x)^*$] = $\stx{foreach}(v\in \stx{scanObj}(??))\{[x]\}$
      \subitem $[xy] = [x]\times[y]$
      \subitem [(x)?] = $\{\stx{if}(??)\{x'\} \;|\; x'\in[x]\}$
     % \subitem [$\demo{\mathcal{S}_l}$] = $\stx{let}v:= \stx{getNth}(\stx{scanLoc}(??),??)$
      %\subitem [$\demo{\mathcal{S}_o}$] = $\stx{let}v:= \stx{getNth}(\stx{scanObj}(??),??)$
      \subitem [$\{\demo{\mathcal{G}_{\tau_l}}$] = $\stx{goto(??:\tau_l)}\}$
      \subitem [$\{\demo{\mathcal{A}_{a,\tau_o}}$] = $\stx{actUnary}(a,??:\tau_o)\}$
      \subitem [$\demo{\mathcal{A}_{a,\tau_{o1},\tau_{o2}}}$] = $\{\stx{actBinary}(a,??:\tau_{o1}, ??:\tau_{o2})\}$
\end{itemize}




\subsection{Sketch Completion Algorithm} % the full details will be presented in section 5

\begin{itemize}
    \item Sketch infeasiblity  
    \subitem we have a sketch S (some holes are remaining from the initial sketch that inferred). At some point during completion we decide to throw S away. Why? 
    \subitem We evaluate S on one of the given demo envs. The result is a partial trace, because at some point execution is going to throw exception, because there holes in the program. 
    \subitem 

    
    \item Sketch prioritization? 
    \
    
\end{itemize}







\newpage
